Photo-chemo-dynamical analysis and the origin of the bulge globular cluster Palomar 6

Palomar 6 (Pal~6) is a moderately metal-poor globular cluster projected towards the Galactic bulge. A full analysis of the cluster can give hints on the early chemical enrichment of the Galaxy and a plausible origin of the cluster. The aim of this study is threefold: a detailed analysis of high-resolution spectroscopic data obtained with the UVES spectrograph at the Very Large Telescope (VLT) at ESO, the derivation of the age and distance of Pal~6 from Hubble Space Telescope (HST) photometric data, and an orbital analysis to determine the probable origin of the cluster. High-resolution spectra of six red giant stars in the direction of Palomar 6 were obtained at the $8$m VLT UT2-Kueyen telescope equipped with the UVES spectrograph in FLAMES$+$UVES configuration. Spectroscopic parameters were derived through excitation and ionisation equilibrium of \ion{Fe}{I} and \ion{Fe}{II} lines, and the abundances were obtained from spectrum synthesis. From HST photometric data, the age and distance were derived through a statistical isochrone fitting. Finally, a dynamical analysis was carried out for the cluster assuming two different Galactic potentials. Four stars that are members of Pal~6 were identified in the sample, which gives a mean radial velocity of $174.3\pm1.6$ km\,s$^{-1}$ and a mean metallicity of [Fe/H]$\,=-1.10\pm0.09$ for the cluster. We found an enhancement of $\alpha$-elements (O, Mg, Si, and Ca) $0.29<\,$[X/Fe]$\,<0.38$ and the iron-peak element Ti of [Ti/Fe]$\,\sim+0.3$. The odd-Z elements (Na and Al) show a mild enhancement of [X/Fe]$\,\sim +0.25$. The abundances of both first- (Y and Zr) and second-peak (Ba and La) heavy elements are relatively high, with $+0.4<\,$[X/Fe]$\,<+0.60$ and $+0.4<\,$[X/Fe]$\,<+0.5$, respectively. The r-element Eu is also relatively high with [Eu/Fe]$\,\sim +0.6$. $\mathbf{\left[Truncated\right]}$

==> feh_ews.tex <==
\onecolumn
\begin{longtable}{lcccccccccc}
\caption{Equivalent widths for \ion{Fe}{I} and \ion{Fe}{II} lines.}            
\label{tab:fe}\\      
\hline
\multirow{2}{*}{Ion} & $\lambda$ & $\chi_{ex}$  & \multirow{2}{*}{log$gf$} &    star 730   &    star 243   &    star 030   &    star 785   &     star 145  &  star 401 \\ 
                     &  [$\AA$]  &  [eV]        &                          & \multicolumn{6}{c}{[m$\AA$]}\\ 
\hline\hline \endfirsthead
\multicolumn{10}{c}%
{{\bfseries \tablename\ \thetable{} -- continued}} \\ \hline
Ion & $\lambda$ & $\chi_{ex}$  & log$gf$ &    star 730   &    star 243   &    star 030   &    star 785   &     star 145  &   star 401 \\ 
%    &  [$\AA$]  &  [eV]        &         & [m$\AA$] & [m$\AA$] & [m$\AA$] & [m$\AA$] & [m$\AA$] & [m$\AA$] \\ 
\hline\hline \endhead

\ion{Fe}{II} & $5991.38$ & $3.15$ & $-3.65$ &    $32.60$  & $39.20$  & $25.5$  &   ---   & $32.3$  &   ---    \\
\ion{Fe}{II} & $6084.11$ & $3.20$ & $-3.97$ &    $35.20$  & $26.20$  & $25.6$  & $28.7$  & $14.3$  & $18.70$  \\
\ion{Fe}{II} & $6149.25$ & $3.89$ & $-2.69$ &    $63.80$  & $43.50$  & $22.3$  & $31.1$  & $24.0$  &   ---    \\
\ion{Fe}{II} & $6247.56$ & $3.89$ & $-2.52$ &      ---    &   ---    & $27.3$  & $25.9$  & $49.4$  & $35.20$  \\
\ion{Fe}{II} & $6416.93$ & $3.89$ & $-2.64$ &    $68.90$  & $36.90$  & $27.1$  &   ---   & $35.4$  & $29.10$  \\
\ion{Fe}{II} & $6432.68$ & $2.89$ & $-3.57$ &    $22.70$  & $31.90$  & $10.2$  & $34.7$  & $28.3$  & $30.10$  \\
\ion{Fe}{II} & $6456.39$ & $3.90$ & $-2.31$ &      ---    & $37.30$  & $29.6$  & $23.3$  & $47.4$  & $54.00$  \\
\ion{Fe}{II} & $6516.08$ & $2.89$ & $-3.31$ &    $62.20$  & $59.2$   & $30.8$  & $43.1$  & $26.7$  & $47.80$  \\
\hline                                  
\ion{Fe}{I} & $5902.48$ & $4.59$ & $-1.81$ &      ---    & $5.10$   & $2.6$   &   ---   & $8.7$   &   ---    \\
\ion{Fe}{I} & $5905.67$ & $4.65$ & $-0.73$ &    $40.90$  &   ---    & $28.5$  &   ---   & $31.9$  &   ---    \\
\ion{Fe}{I} & $5905.69$ & $4.65$ & $-0.73$ &      ---    & $40.60$  &   ---   & $46.7$  &   ---   & $43.90$  \\
\ion{Fe}{I} & $5909.97$ & $3.21$ & $-2.78$ &      ---    & $84.90$  &   ---   & $32.7$  &   ---   & $59.80$  \\
\ion{Fe}{I} & $5916.25$ & $2.45$ & $-2.97$ &    $59.50$  &   ---    &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $5916.26$ & $2.45$ & $-2.99$ &      ---    & $91.10$  & $30.9$  & $25.1$  & $32.0$  & $72.10$  \\
\ion{Fe}{I} & $5927.79$ & $4.65$ & $-1.09$ &    $38.50$  & $37.70$  & $44.4$  & $46.7$  &   ---   &   ---    \\
\ion{Fe}{I} & $5929.67$ & $4.55$ & $-1.41$ &    $45.50$  & $44.90$  & $31.3$  &   ---   &   ---   & $30.70$  \\
\ion{Fe}{I} & $5930.18$ & $4.65$ & $-0.23$ &    $51.70$  &   ---    &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $5930.19$ & $4.65$ & $-0.23$ &      ---    & $78.70$  &   ---   & $68.3$  &   ---   & $68.70$  \\
\ion{Fe}{I} & $5934.65$ & $3.93$ & $-1.17$ &    $34.30$  &   ---    & $54.0$  &   ---   & $70.4$  &   ---    \\
\ion{Fe}{I} & $5934.67$ & $3.93$ & $-1.17$ &      ---    & $76.40$  &   ---   & $28.8$  &   ---   & $62.30$  \\
\ion{Fe}{I} & $5952.73$ & $3.98$ & $-1.44$ &    $48.50$  & $50.40$  &   ---   & $30.8$  & $52.7$  & $40.10$  \\
\ion{Fe}{I} & $5956.69$ & $0.86$ & $-4.60$ &    $42.10$  &   ---    & $37.5$  &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $5956.71$ & $0.86$ & $-4.61$ &      ---    & $79.10$  &   ---   &   ---   &   ---   & $82.50$  \\
\ion{Fe}{I} & $5975.35$ & $4.84$ & $-0.69$ &    $36.80$  &   ---    & $15.6$  &   ---   & $42.3$  &   ---    \\
\ion{Fe}{I} & $5983.69$ & $4.55$ & $-1.47$ &    $30.80$  & $52.80$  & $17.2$  &   ---   & $20.1$  & $43.90$  \\
\ion{Fe}{I} & $5987.06$ & $4.80$ & $-0.43$ &    $43.30$  &   ---    & $27.0$  &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $5987.07$ & $4.79$ & $-0.15$ &      ---    & $62.90$  &   ---   &   ---   &   ---   & $59.60$  \\
\ion{Fe}{I} & $6003.01$ & $3.88$ & $-1.12$ &    $44.80$  &   ---    &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6003.02$ & $3.88$ & $-1.12$ &      ---    & $90.40$  & $25.4$  & $44.3$  & $63.7$  & $76.00$  \\
\ion{Fe}{I} & $6005.54$ & $2.59$ & $-3.61$ &    $40.50$  &   ---    & $34.4$  &   ---   & $43.6$  &   ---    \\
\ion{Fe}{I} & $6008.56$ & $3.88$ & $-0.99$ &    $31.50$  &   ---    & $25.3$  &   ---   & $57.2$  &   ---    \\
\ion{Fe}{I} & $6020.17$ & $4.61$ & $-0.27$ &    $38.10$  &   ---    & $29.2$  &   ---   & $64.5$  &   ---    \\
\ion{Fe}{I} & $6024.05$ & $4.55$ & $-0.12$ &    $31.20$  & $90.40$  & $2.00$  & $73.9$  & $45.0$  & $69.90$  \\
\ion{Fe}{I} & $6027.06$ & $4.08$ & $-1.09$ &    $80.00$  & $79.70$  & $29.7$  & $43.2$  & $32.5$  & $59.10$  \\
\ion{Fe}{I} & $6054.08$ & $4.37$ & $-2.31$ &    $46.50$  & $16.50$  &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6056.01$ & $4.73$ & $-0.46$ &      ---    & $62.30$  & $35.7$  & $41.9$  & $23.8$  & $41.70$  \\
\ion{Fe}{I} & $6065.48$ & $2.61$ & $-1.53$ &    $66.00$  &   ---    &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6065.49$ & $2.61$ & $-1.53$ &      ---    & $132.60$ &   ---   &   ---   &   ---   & $101.5$  \\
\ion{Fe}{I} & $6078.49$ & $4.80$ & $-0.32$ &    $57.70$  &   ---    &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6078.50$ & $4.79$ & $-0.40$ &      ---    & $65.90$  & $18.0$  & $49.5$  & $41.5$  & $65.40$  \\
\ion{Fe}{I} & $6079.00$ & $4.65$ & $-1.13$ &      ---    &   ---    &   ---   &   ---   & $44.2$  & $36.90$  \\
\ion{Fe}{I} & $6079.01$ & $4.65$ & $-1.12$ &    $57.10$  &   ---    &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6082.71$ & $2.22$ & $-3.57$ &    $31.20$  &   ---    &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6082.72$ & $2.22$ & $-3.57$ &      ---    & $69.20$  &   ---   & $72.2$  &   ---   & $65.10$  \\
\ion{Fe}{I} & $6093.64$ & $4.61$ & $-1.50$ &    $25.10$  &   ---    & $11.3$  &   ---   & $41.9$  &   ---    \\
\ion{Fe}{I} & $6093.67$ & $4.60$ & $-1.51$ &      ---    & $15.50$  &   ---   &   ---   &   ---   & $25.70$  \\
\ion{Fe}{I} & $6094.36$ & $4.65$ & $-1.94$ &    $46.10$  & $18.80$  &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6096.66$ & $3.98$ & $-1.93$ &      ---    & $43.00$  &   ---   & $39.1$  &   ---   &   ---    \\
\ion{Fe}{I} & $6105.15$ & $4.54$ & $-2.07$ &      ---    & $16.50$  &   ---   &   ---   &   ---   & $10.40$  \\
\ion{Fe}{I} & $6137.70$ & $2.59$ & $-1.40$ &    $40.00$  & $142.10$ &   ---   &   ---   &   ---   & $146.5$  \\
\ion{Fe}{I} & $6151.62$ & $2.18$ & $-3.30$ &    $59.50$  & $114.00$ & $56.4$  & $48.4$  & $37.3$  & $110.8$  \\
\ion{Fe}{I} & $6157.73$ & $4.08$ & $-1.25$ &      ---    & $67.10$  & $27.9$  & $37.8$  & $35.1$  & $58.30$  \\
\ion{Fe}{I} & $6159.38$ & $4.61$ & $-1.97$ &    $26.40$  &   ---    &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6165.36$ & $4.14$ & $-1.47$ &    $43.50$  & $64.90$  & $43.1$  &   ---   & $17.7$  &   ---    \\
\ion{Fe}{I} & $6173.34$ & $2.22$ & $-2.88$ &      ---    & $122.80$ &   ---   & $46.9$  &   ---   & $96.80$  \\
\ion{Fe}{I} & $6180.21$ & $2.73$ & $-2.59$ &    $56.30$  & $89.50$  & $36.3$  &   ---   & $58.5$  & $63.90$  \\
\ion{Fe}{I} & $6187.99$ & $3.94$ & $-1.72$ &    $63.80$  & $60.10$  & $34.2$  & $48.4$  &   ---   & $62.90$  \\
\ion{Fe}{I} & $6200.32$ & $2.61$ & $-2.44$ &      ---    & $88.40$  &   ---   &   ---   &   ---   & $80.40$  \\
\ion{Fe}{I} & $6213.44$ & $2.22$ & $-2.48$ &    $88.90$  & $129.90$ & $39.5$  &   ---   &   ---   & $105.50$ \\
\ion{Fe}{I} & $6219.29$ & $2.20$ & $-2.43$ &    $96.80$  & $134.10$ &   ---   &   ---   &   ---   & $116.50$ \\
\ion{Fe}{I} & $6220.78$ & $3.88$ & $-2.46$ &    $65.00$  &   ---    &   ---   &   ---   &   ---   & $24.60$  \\
\ion{Fe}{I} & $6226.73$ & $3.88$ & $-2.22$ &    $47.40$  & $32.00$  &   ---   & $18.4$  &   ---   &   ---    \\
\ion{Fe}{I} & $6229.23$ & $2.84$ & $-2.97$ &      ---    & $83.70$  & $11.7$  & $58.5$  & $31.3$  & $52.30$  \\
\ion{Fe}{I} & $6240.65$ & $2.22$ & $-3.21$ &      ---    & $97.30$  & $17.9$  & $44.6$  & $40.6$  & $77.20$  \\
\ion{Fe}{I} & $6246.33$ & $3.60$ & $-0.88$ &      ---    & $34.30$  &   ---   & $89.4$  &   ---   & $87.30$  \\
\ion{Fe}{I} & $6252.57$ & $2.40$ & $-1.69$ &    $54.20$  & $162.20$ &   ---   & $137.8$ &   ---   & $110.40$ \\
\ion{Fe}{I} & $6254.25$ & $2.28$ & $-2.44$ &    $24.30$  &   ---    &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6265.14$ & $2.18$ & $-2.55$ &    $61.90$  & $119.90$ &   ---   & $121.9$ &   ---   & $105.40$ \\
\ion{Fe}{I} & $6270.23$ & $2.86$ & $-2.46$ &    $36.70$  & $61.10$  & $21.2$  & $32.4$  & $90.8$  & $61.50$  \\
\ion{Fe}{I} & $6271.28$ & $3.32$ & $-2.70$ &    $23.20$  & $40.70$  & $19.0$  & $36.4$  & $24.6$  & $39.70$  \\
\ion{Fe}{I} & $6297.80$ & $2.22$ & $-2.74$ &      ---    & $130.10$ &   ---   & $58.6$  & $84.8$  & $101.60$ \\
\ion{Fe}{I} & $6301.51$ & $3.65$ & $-0.72$ &    $138.40$ & $118.20$ &   ---   & $127.7$ &   ---   &   ---    \\
\ion{Fe}{I} & $6302.50$ & $3.69$ & $-0.91$ &      ---    & $94.40$  &   ---   & $148.5$ &   ---   &   ---    \\
\ion{Fe}{I} & $6311.50$ & $2.83$ & $-3.14$ &    $85.60$  & $81.20$  &   ---   & $26.2$  & $63.2$  & $36.50$  \\
\ion{Fe}{I} & $6315.31$ & $4.14$ & $-1.23$ &    $51.70$  & $79.10$  & $5.7$   & $42.9$  & $25.1$  & $53.60$  \\
\ion{Fe}{I} & $6315.81$ & $4.08$ & $-1.71$ &    $35.30$  & $48.60$  & $22.4$  & $58.1$  & $37.2$  & $50.10$  \\
\ion{Fe}{I} & $6322.69$ & $2.59$ & $-2.43$ &      ---    & $80.80$  &   ---   & $36.9$  &   ---   & $92.80$  \\
\ion{Fe}{I} & $6330.84$ & $4.73$ & $-1.74$ &      ---    & $44.60$  &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6335.34$ & $2.20$ & $-2.18$ &    $43.4$   & $143.30$ & $1.5$   & $88.4$  &   ---   & $119.30$ \\
\ion{Fe}{I} & $6336.83$ & $3.69$ & $-1.05$ &      ---    & $105.70$ & $38.7$  & $84.5$  & $60.5$  & $102.80$ \\
\ion{Fe}{I} & $6344.16$ & $2.43$ & $-2.92$ &    $87.20$  & $127.10$ & $22.8$  & $75.8$  & $82.3$  & $90.70$  \\
\ion{Fe}{I} & $6355.04$ & $2.84$ & $-2.29$ &      ---    & $128.30$ &   ---   &   ---   &   ---   & $92.70$  \\
\ion{Fe}{I} & $6358.69$ & $0.86$ & $-4.47$ &      ---    & $160.90$ &   ---   &   ---   &   ---   & $149.70$ \\
\ion{Fe}{I} & $6380.75$ & $4.19$ & $-1.38$ &    $50.80$  & $42.00$  & $15.9$  & $23.8$  & $36.2$  & $50.30$  \\
\ion{Fe}{I} & $6392.54$ & $2.28$ & $-4.03$ &    $52.50$  & $63.10$  & $11.7$  &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6393.61$ & $2.43$ & $-1.43$ &    $46.5$   & $158.70$ &   ---   &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6408.03$ & $3.69$ & $-1.00$ &      ---    & $101.50$ &   ---   &   ---   & $74.9$  & $95.80$  \\
\ion{Fe}{I} & $6411.11$ & $4.73$ & $-1.92$ &    $40.10$  & $13.70$  &   ---   &   ---   &   ---   & $5.0$    \\
\ion{Fe}{I} & $6411.66$ & $3.65$ & $-0.60$ &    $48.50$  & $121.10$ &   ---   &   ---   & $105.$  & $98.70$  \\
\ion{Fe}{I} & $6419.94$ & $4.73$ & $-0.24$ &    $44.40$  & $78.70$  & $15.6$  & $75.9$  & $44.2$  & $80.60$  \\
\ion{Fe}{I} & $6421.35$ & $2.28$ & $-2.03$ &    $71.10$  & $158.20$ &   ---   &   ---   & $107.$  & $113.50$ \\
\ion{Fe}{I} & $6430.86$ & $2.18$ & $-2.01$ &    $51.30$  & $174.20$ &   ---   &   ---   &   ---   & $123.40$ \\
\ion{Fe}{I} & $6469.21$ & $4.83$ & $-0.77$ &    $73.50$  & $84.00$  &   ---   & $56.5$  & $27.7$  &   ---    \\
\ion{Fe}{I} & $6475.63$ & $2.56$ & $-2.94$ &    $63.00$  & $127.30$ & $18.3$  & $70.5$  & $31.2$  &   ---    \\
\ion{Fe}{I} & $6481.88$ & $2.28$ & $-2.98$ &      ---    & $140.40$ & $16.6$  & $55.1$  & $70.5$  & $97.50$  \\
\ion{Fe}{I} & $6494.99$ & $2.40$ & $-1.27$ &    $143.20$ &   ---    & $57.1$  &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6498.95$ & $0.96$ & $-4.70$ &      ---    & $123.10$ &   ---   & $33.8$  &   ---   & $109.60$ \\
\ion{Fe}{I} & $6518.37$ & $2.83$ & $-2.30$ &      ---    & $83.60$  &   ---   & $51.1$  &   ---   & $81.30$  \\
\ion{Fe}{I} & $6533.93$ & $4.56$ & $-1.45$ &      ---    & $31.30$  & $2.00$  &   ---   & $29.5$  &   ---    \\
\ion{Fe}{I} & $6546.25$ & $2.75$ & $-1.54$ &    $106.10$ & $159.90$ & $63.3$  &   ---   &   ---   & $141.80$ \\
\ion{Fe}{I} & $6556.81$ & $4.79$ & $-1.72$ &      ---    & $19.00$  &   ---   & $28.1$  &   ---   &   ---    \\
\ion{Fe}{I} & $6569.22$ & $4.73$ & $-0.42$ &    $99.40$  & $77.60$  & $31.6$  &   ---   & $55.9$  & $69.30$  \\
\ion{Fe}{I} & $6574.25$ & $0.99$ & $-5.02$ &      ---    & $116.30$ &   ---   & $26.7$  &   ---   & $93.60$  \\
\ion{Fe}{I} & $6575.04$ & $2.59$ & $-2.71$ &      ---    & $121.80$ &   ---   &   ---   &   ---   & $80.90$  \\
\ion{Fe}{I} & $6581.21$ & $1.48$ & $-4.68$ &    $85.20$  & $97.20$  &   ---   & $32.0$  & $23.1$  & $65.70$  \\
\ion{Fe}{I} & $6591.31$ & $4.59$ & $-2.07$ &    $28.10$  & $10.70$  & $1.00$  &   ---   &   ---   & $11.50$  \\
\ion{Fe}{I} & $6593.87$ & $2.43$ & $-2.42$ &    $39.60$  & $136.20$ & $69.4$  &   ---   &   ---   & $103.70$ \\
\ion{Fe}{I} & $6597.56$ & $4.80$ & $-1.07$ &    $45.70$  & $36.50$  & $26.7$  &   ---   &   ---   & $36.00$  \\
\ion{Fe}{I} & $6608.04$ & $2.28$ & $-4.03$ &    $74.30$  & $62.60$  & $10.0$  &   ---   & $49.4$  & $45.40$  \\
\ion{Fe}{I} & $6609.12$ & $2.56$ & $-2.69$ &    $73.40$  & $132.60$ & $24.5$  & $73.0$  &   ---   & $131.60$ \\
\ion{Fe}{I} & $6627.54$ & $4.55$ & $-1.68$ &    $36.80$  & $42.40$  & $5.1$   &   ---   & $9.9$   &   ---    \\
\ion{Fe}{I} & $6678.00$ & $2.69$ & $-1.42$ &    $45.00$  & $157.60$ &   ---   &   ---   &   ---   & $118.10$ \\
\ion{Fe}{I} & $6699.14$ & $4.59$ & $-2.10$ &    $24.40$  & $24.20$  & $2.70$  &   ---   &   ---   &   ---    \\
\ion{Fe}{I} & $6705.11$ & $4.61$ & $-1.06$ &      ---    &   ---    & $16.3$  &   ---   & $30.8$  &   ---    \\
\ion{Fe}{I} & $6726.67$ & $4.59$ & $-1.09$ &      ---    &   ---    & $28.0$  &   ---   & $16.0$  &   ---    \\
 \\ \hline \hline \\            
\end{longtable} 
\twocolumn

==> line_abundances.tex <==
\clearpage
\onecolumn
\begin{landscape}
\begin{table*}
\centering
\caption{Line-by-line abundances ratios in the six UVES sample stars for the CNO, odd-Z (Na and Al), alpha- (Mg, Si, Ca, and Ti), and heavy-elements (Y, Zr, Ba, La, and Eu).}            
\label{tab:lines_ratios}   
\small
\scalefont{0.9}
%\centering
\tabcolsep 0.15cm
\begin{tabular}{lccccccccc|lccccccccc}
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\multirow{2}{*}{Species} & $\lambda$    & \phantom{-}\phantom{-}{ $\chi_{ex}$ }&  \multirow{2}{*}{log$gf$} & \multicolumn{6}{c}{[X/Fe]} & \multirow{2}{*}{Species} & $\lambda$    & \phantom{-}\phantom{-}{ $\chi_{ex}$ }&  \multirow{2}{*}{log$gf$} & \multicolumn{6}{c}{[X/Fe]}\\
                         & [$\AA$]      &    [eV]      &                           & star 730 & star 243 & star 030 & star 785 &  star 145 & star 401 &                          & [$\AA$]      &    [eV]      &                           & star 730 & star 243 & star 030 & star 785 &  star 145 & star 401 \\ \hline\hline

\ion{Na}{I}   &  $5682.633$  &  $2.10$  &  $-0.71$  &  $+0.07$  &  $+0.28$  &  $-0.09$  &  $+0.27$  &  ---      &  ---      & \ion{Ti}{I}   &  $5922.108$  &  $1.05$  &  $-1.46$  &  ---      &  $+0.43$  &  $+0.32$  &  $+0.40$  &  $+0.27$  &  $+0.35$  \\
\ion{Na}{I}   &  $6154.230$  &  $2.10$  &  $-1.56$  &  ---      &  $+0.48$  &  $+0.43$  &  $+0.42$  &  $+0.42$  &  ---      & \ion{Ti}{I}   &  $5941.750$  &  $1.05$  &  $-1.50$  &  $+0.49$  &  $+0.28$  &  $+0.50$  &  $+0.30$  &  $+0.23$  &  $+0.35$  \\
\ion{Na}{I}   &  $6160.753$  &  $2.10$  &  $-1.26$  &  $+0.51$  &  $+0.51$  &  ---      &  $+0.13$  &  $+0.37$  &  $+0.10$  & \ion{Ti}{I}   &  $5965.825$  &  $1.88$  &  $-0.42$  &  $+0.54$  &  $+0.53$  &  $+0.47$  &  $+0.20$  &  $+0.30$  &  $+0.33$  \\
\ion{Al}{I}   &  $6696.185$  &  $4.02$  &  $-1.58$  &  $+0.47$  &  $+0.37$  &  $+0.59$  &  $+0.09$  &  $+0.08$  &  $+0.33$  & \ion{Ti}{I}   &  $5978.539$  &  $1.87$  &  $-0.53$  &  $+0.02$  &  $+0.36$  &  $+0.46$  &  $+0.60$  &  $+0.56$  &  $+0.13$  \\
\ion{Al}{I}   &  $6698.673$  &  $3.14$  &  $-1.65$  &  $+0.42$  &  $+0.14$  &  $+0.39$  &  $+0.29$  &  $+0.15$  &  $+0.47$  & \ion{Ti}{I}   &  $6064.623$  &  $1.05$  &  $-1.94$  &  ---      &  $+0.58$  &  $+0.48$  &  ---      &  $+0.44$  &  $+0.35$  \\
\ion{Mg}{I}   &  $5528.405$  &  $5.11$  &  $-2.10$  &  ---      &  ---      &  ---      &  $+0.14$  &  ---      &  ---      & \ion{Ti}{I}   &  $6091.169$  &  $2.27$  &  $-0.42$  &  $+0.36$  &  $+0.43$  &  $+0.49$  &  $+0.40$  &  $+0.49$  &  $+0.33$  \\
\ion{Mg}{I}   &  $6318.720$  &  $5.11$  &  $-2.36$  &  $+0.41$  &  $+0.48$  &  $+0.58$  &  $+0.34$  &  $+0.49$  &  $+0.24$  & \ion{Ti}{I}   &  $6126.214$  &  $1.07$  &  $-1.43$  &  $+0.46$  &  $+0.57$  &  $+0.36$  &  $+0.00$  &  $+0.33$  &  $+0.22$  \\
\ion{Mg}{I}   &  $6319.242$  &  $5.11$  &  $-2.80$  &  $+0.45$  &  $+0.45$  &  $+0.53$  &  ---      &  $+0.40$  &  $+0.40$  & \ion{Ti}{I}   &  $6258.110$  &  $1.44$  &  $-0.36$  &  $+0.11$  &  $+0.31$  &  $+0.22$  &  $+0.00$  &  $-0.08$  &  $-0.22$  \\  
\ion{Mg}{I}   &  $6765.450$  &  $5.75$  &  $-1.94$  &  ---      &  $+0.27$  &  $+0.47$  &  $+0.27$  &  $+0.55$  &  $+0.25$  & \ion{Ti}{I}   &  $6261.106$  &  $1.43$  &  $-0.48$  &  $+0.57$  &  $+0.45$  &  $+0.13$  &  $+0.00$  &  $-0.04$  &  $+0.06$  \\  
\ion{Si}{I}   &  $5665.555$  &  $4.92$  &  $-2.04$  &  $+0.48$  &  $+0.19$  &  $+0.38$  &  $+0.60$  &  $+0.51$  &  $+0.61$  & \ion{Ti}{I}   &  $6303.767$  &  $1.44$  &  $-1.57$  &  $+0.56$  &  $+0.56$  &  ---      &  $+0.20$  &  $+0.57$  &  $+0.39$  \\
\ion{Si}{I}   &  $5666.690$  &  $5.62$  &  $-1.74$  &  $+0.41$  &  $+0.59$  &  $+0.50$  &  $+0.20$  &  ---      &  $+0.44$  & \ion{Ti}{I}   &  $6312.240$  &  $1.46$  &  $-1.60$  &  ---      &  ---      &  $+0.09$  &  $+0.50$  &  ---      &  $+0.26$  \\
\ion{Si}{I}   &  $5690.425$  &  $4.93$  &  $-1.87$  &  $+0.07$  &  $+0.58$  &  $+0.12$  &  ---      &  $+0.43$  &  $+0.60$  & \ion{Ti}{I}   &  $6336.113$  &  $1.44$  &  $-1.74$  &  ---      &  $+0.25$  &  ---      &  ---      &  ---      &  $+0.56$  \\ 
\ion{Si}{I}   &  $5948.545$  &  $5.08$  &  $-1.30$  &  $+0.21$  &  $+0.18$  &  $+0.13$  &  $+0.15$  &  $+0.54$  &  $+0.39$  & \ion{Ti}{I}   &  $6508.150$  &  $1.43$  &  $-2.05$  &  ---      &  $+0.60$  &  ---      &  ---      &  ---      &  $+0.28$  \\
\ion{Si}{I}   &  $6142.494$  &  $5.62$  &  $-1.50$  &  $+0.24$  &  $+0.22$  &  ---      &  $+0.50$  &  $+0.02$  &  $+0.29$  & \ion{Ti}{I}   &  $6554.238$  &  $1.44$  &  $-1.22$  &  $-0.10$  &  $+0.47$  &  $+0.33$  &  $+0.20$  &  $+0.37$  &  $+0.38$  \\
\ion{Si}{I}   &  $6145.020$  &  $5.61$  &  $-1.45$  &  $+0.49$  &  $+0.19$  &  ---      &  ---      &  $+0.23$  &  $+0.42$  & \ion{Ti}{I}   &  $6556.077$  &  $1.46$  &  $-1.07$  &  $+0.25$  &  ---      &  $+0.42$  &  $+0.40$  &  $+0.46$  &  $+0.59$  \\
\ion{Si}{I}   &  $6155.142$  &  $5.62$  &  $-0.85$  &  $+0.05$  &  $+0.40$  &  $+0.20$  &  $+0.30$  &  $+0.09$  &  $+0.25$  & \ion{Ti}{I}   &  $6599.113$  &  $0.90$  &  $-2.09$  &  $+0.52$  &  $+0.50$  &  $+0.46$  &  $+0.60$  &  $+0.68$  &  $+0.40$  \\
\ion{Si}{I}   &  $6237.328$  &  $5.61$  &  $-1.01$  &  $+0.43$  &  $+0.48$  &  $+0.31$  &  $+0.29$  &  $+0.43$  &  $+0.48$  & \ion{Ti}{I}   &  $6743.127$  &  $0.90$  &  $-1.73$  &  $+0.39$  &  $+0.47$  &  $+0.10$  &  $+0.40$  &  $+0.49$  &  $+0.52$  \\
\ion{Si}{I}   &  $6243.823$  &  $5.61$  &  $-1.30$  &  $+0.53$  &  $+0.46$  &  ---      &  $+0.42$  &  $+0.46$  &  $+0.06$  & \ion{Ti}{II}  &  $5418.751$  &  $1.58$  &  $-2.13$  &  ---      &  ---      &  $-0.23$  &  ---      &  $+0.20$  &  $+0.27$  \\
\ion{Si}{I}   &  $6414.987$  &  $5.87$  &  $-1.13$  &  $+0.12$  &  $+0.45$  &  $+0.42$  &  $+0.51$  &  $+0.67$  &  $+0.64$  & \ion{Ti}{II}  &  $6491.580$  &  $2.06$  &  $-2.10$  &  $+0.18$  &  $+0.38$  &  $+0.23$  &  $-0.10$  &  $+0.00$  &  $+0.41$  \\
\ion{Si}{I}   &  $6721.844$  &  $5.86$  &  $-1.17$  &  $+0.60$  &  $+0.43$  &  $+0.52$  &  $+0.49$  &  $+0.40$  &  $+0.31$  & \ion{Ti}{II}  &  $6559.576$  &  $2.05$  &  $-2.35$  &  $+0.14$  &  $+0.26$  &  $+0.48$  &  $+0.10$  &  $+0.26$  &  ---      \\
\ion{Ca}{I}   &  $5601.277$  &  $2.53$  &  $-0.52$  &  $-0.33$  &  $+0.07$  &  ---      &  ---      &  ---      &  $+0.22$  & \ion{Ti}{II}  &  $6606.970$  &  $2.06$  &  $-2.85$  &  $+0.26$  &  $+0.39$  &  $+0.02$  &  $+0.40$  &  $+0.36$  &  $+0.23$  \\    
\ion{Ca}{I}   &  $5867.562$  &  $2.93$  &  $-1.55$  &  $+0.50$  &  $+0.02$  &  $+0.49$  &  $+0.40$  &  $+0.41$  &  $+0.40$  & \ion{Y}{I}    &  $6435.004$  &  $0.07$  &  $-0.82$  &  $+0.02$  &  $+0.44$  &  $+1.12$  &  $+0.78$  &  $+0.89$  &  $-0.01$ \\
\ion{Ca}{I}   &  $6156.030$  &  $2.52$  &  $-2.39$  &  ---      &  ---      &  ---      &  $+0.40$  &  $+0.56$  &  $+0.44$  & \ion{Y}{II}   &  $6795.414$  &  $1.74$  &  $-1.19$  &  $+0.33$  &  $+0.23$  &  $+0.48$  &  $+0.84$  &  $+0.57$  &  $+0.09$ \\ 
\ion{Ca}{I}   &  $6161.295$  &  $2.51$  &  $-1.02$  &  $+0.26$  &  ---      &  $+0.50$  &  $-0.10$  &  $-0.09$  &  $+0.48$  & \ion{Zr}{I}   &  $6127.475$  &  $0.15$  &  $-1.06$  &  $+0.71$  &  $+0.74$  &  $+0.58$  &  $+0.60$  &  $+0.85$  &  $+0.29$ \\
\ion{Ca}{I}   &  $6166.440$  &  $2.52$  &  $-0.90$  &  $+0.37$  &  $+0.53$  &  $-0.39$  &  $+0.30$  &  $+0.27$  &  $+0.11$  & \ion{Zr}{I}   &  $6134.585$  &  $0.00$  &  $-1.42$  &  $+0.86$  &  $+0.37$  &  $+0.84$  &   ---     &  $+0.33$  &  $+0.48$ \\
\ion{Ca}{I}   &  $6169.044$  &  $2.52$  &  $-0.54$  &  $+0.45$  &  $+0.43$  &  ---      &  $+0.00$  &  $+0.11$  &  $+0.28$  & \ion{Zr}{I}   &  $6140.535$  &  $0.52$  &  $-1.60$  &   ---     &  $+0.86$  &   ---     &   ---     &  $+0.95$  &  $+0.92$ \\
\ion{Ca}{I}   &  $6169.564$  &  $2.52$  &  $-0.27$  &  $+0.55$  &  $+0.44$  &  ---      &  ---      &  $+0.15$  &  $+0.42$  & \ion{Zr}{I}   &  $6143.252$  &  $0.07$  &  $-1.10$  &  $+0.71$  &  $+0.75$  &  $+0.54$  &  $+0.63$  &  $+0.84$  &  $-0.04$ \\
\ion{Ca}{I}   &  $6439.080$  &  $2.52$  &  $+0.30$  &  $+0.24$  &  $+0.55$  &  ---      &  ---      &  ---      &  $+0.50$  & \ion{Ba}{II}  &  $5853.675$  &  $0.60$  &  $-1.10$  &   ---     &  $+0.52$  &   ---     &   ---     &   ---     &  $+0.36$ \\  
\ion{Ca}{I}   &  $6455.605$  &  $2.52$  &  $-1.35$  &  $+0.47$  &  $+0.48$  &  $+0.43$  &  $+0.10$  &  $+0.40$  &  $+0.47$  & \ion{Ba}{II}  &  $6496.897$  &  $0.60$  &  $-0.32$  &   ---     &  $+0.65$  &   ---     &  $+0.23$  &   ---     &  $+0.62$ \\
\ion{Ca}{I}   &  $6464.679$  &  $2.52$  &  $-2.10$  &  ---      &  ---      &  ---      &  $+0.49$  &  $+0.37$  &  $+0.55$  & \ion{La}{II}  &  $6172.721$  &  $0.13$  &  $-2.25$  &  $+0.72$  &  $+0.03$  &  $+0.86$  &  $+0.78$  &  $+0.81$  &  $+0.32$ \\
\ion{Ca}{I}   &  $6493.788$  &  $2.52$  &  $-2.44$  &  $-0.07$  &  $+0.14$  &  ---      &  ---      &  ---      &  $-0.10$  & \ion{La}{II}  &  $6262.287$  &  $0.40$  &  $-1.60$  &  $+0.55$  &  $+0.30$  &   ---     &   ---     &  $+0.37$  &  $+0.16$ \\  
\ion{Ca}{I}   &  $6499.654$  &  $2.52$  &  $-0.85$  &  $+0.36$  &  $+0.58$  &  $+0.15$  &  ---      &  $+0.20$  &  $+0.43$  & \ion{La}{II}  &  $6296.079$  &  $1.25$  &  $-0.84$  &  $+0.37$  &   ---     &   ---     &   ---     &   ---     &  $+0.19$ \\
\ion{Ca}{I}   &  $6572.779$  &  $0.00$  &  $-4.32$  &  ---      &  ---      &  $-0.16$  &  $+0.20$  &  $+0.32$  &  $+0.08$  & \ion{La}{II}  &  $6320.376$  &  $0.17$  &  $-1.56$  &  $+0.37$  &  $+0.29$  &  $+0.19$  &  $+0.52$  &  $+0.79$  &  $+0.21$ \\
\ion{Ca}{I}   &  $6717.687$  &  $2.71$  &  $-0.61$  &  $+0.46$  &  ---      &  $-0.23$  &  $-0.10$  &  $+0.33$  &  $+0.43$  & \ion{La}{II}  &  $6390.477$  &  $0.32$  &  $-1.41$  &  $+0.31$  &  $+0.10$  &  $+0.67$  &  $+0.77$  &  $+0.75$  &  $+0.30$ \\
\ion{Ti}{I}   &  $5689.459$  &  $2.29$  &  $-0.44$  &  $+0.39$  &  $+0.39$  &  $+0.42$  &  $+0.49$  &  $+0.44$  &  $+0.58$  & \ion{Eu}{II}  &  $6437.640$  &  $1.32$  &  $-0.32$  &  $+0.55$  &  $+0.50$  &  $+0.62$  &  $+0.65$  &  $+0.77$  &  $+0.57$ \\
\ion{Ti}{I}   &  $5866.449$  &  $1.07$  &  $-0.84$  &  $+0.36$  &  $+0.51$  &  $+0.12$  &  $+0.09$  &  $+0.48$  &  $+0.29$  & \ion{Eu}{II}  &  $6645.064$  &  $1.38$  &  $+0.12$  &  $+0.31$  &  $+0.12$  &  $+0.37$  &  $+0.82$  &  $+0.72$  &  $+0.59$ \\


\noalign{\vskip 0.2cm}
\noalign{\hrule}
\noalign{\smallskip} \hline
\end{tabular}
\end{table*}
\end{landscape} 
\clearpage
\normalsize
\twocolumn

==> line_abundances_1column.tex <==
\onecolumn
\begin{longtable}{lccccccccc}
\caption{Line-by-line abundances ratios in the six UVES sample stars for the CNO, odd-Z (Na and Al), alpha- (Mg, Si, Ca, and Ti), and heavy-elements (Y, Zr, Ba, La, and Eu).}            
\label{tab:lines_ratios}\\   
\hline
\noalign{\smallskip}
\multirow{2}{*}{Species} & $\lambda$    & \phantom{-}\phantom{-}{ $\chi_{ex}$ }&  \multirow{2}{*}{log$gf$} &    star 730   &    star 243   &    star 030   &    star 785   &     star 145  &   star 401 \\
                     &  [$\AA$]  &  [eV]        &                          & \multicolumn{6}{c}{[X/Fe]}\\ 
\hline\hline \endfirsthead
\multicolumn{10}{c}%
{{\bfseries \tablename\ \thetable{} -- continued}} \\ \hline
Species & $\lambda$    & \phantom{-}\phantom{-}{ $\chi_{ex}$ }&  log$gf$ &    star 730   &    star 243   &    star 030   &    star 785   &     star 145  &   star 401 \\ 
\hline\hline \endhead

\ion{Na}{I}   &  $5682.633$  &  $2.10$  &  $-0.71$  &  $+0.07$  &  $+0.28$  &  $-0.09$  &  $+0.27$  &  ---      &  ---      \\ 
\ion{Na}{I}   &  $6154.230$  &  $2.10$  &  $-1.56$  &  ---      &  $+0.48$  &  $+0.43$  &  $+0.42$  &  $+0.42$  &  ---      \\
\ion{Na}{I}   &  $6160.753$  &  $2.10$  &  $-1.26$  &  $+0.51$  &  $+0.51$  &  ---      &  $+0.13$  &  $+0.37$  &  $+0.10$  \\
\ion{Al}{I}   &  $6696.185$  &  $4.02$  &  $-1.58$  &  $+0.47$  &  $+0.37$  &  $+0.59$  &  $+0.09$  &  $+0.08$  &  $+0.33$  \\
\ion{Al}{I}   &  $6698.673$  &  $3.14$  &  $-1.65$  &  $+0.42$  &  $+0.14$  &  $+0.39$  &  $+0.29$  &  $+0.15$  &  $+0.47$  \\
\hline
\ion{Mg}{I}   &  $5528.405$  &  $5.11$  &  $-2.10$  &  ---      &  ---      &  ---      &  $+0.14$  &  ---      &  ---      \\ 
\ion{Mg}{I}   &  $6318.720$  &  $5.11$  &  $-2.36$  &  $+0.41$  &  $+0.48$  &  $+0.58$  &  $+0.34$  &  $+0.49$  &  $+0.24$  \\
\ion{Mg}{I}   &  $6319.242$  &  $5.11$  &  $-2.80$  &  $+0.45$  &  $+0.45$  &  $+0.53$  &  ---      &  $+0.40$  &  $+0.40$  \\
\ion{Mg}{I}   &  $6765.450$  &  $5.75$  &  $-1.94$  &  ---      &  $+0.27$  &  $+0.47$  &  $+0.27$  &  $+0.55$  &  $+0.25$  \\
\ion{Si}{I}   &  $5665.555$  &  $4.92$  &  $-2.04$  &  $+0.48$  &  $+0.19$  &  $+0.38$  &  $+0.60$  &  $+0.51$  &  $+0.61$  \\
\ion{Si}{I}   &  $5666.690$  &  $5.62$  &  $-1.74$  &  $+0.41$  &  $+0.59$  &  $+0.50$  &  $+0.20$  &  ---      &  $+0.44$  \\
\ion{Si}{I}   &  $5690.425$  &  $4.93$  &  $-1.87$  &  $+0.07$  &  $+0.58$  &  $+0.12$  &  ---      &  $+0.43$  &  $+0.60$  \\  
\ion{Si}{I}   &  $5948.545$  &  $5.08$  &  $-1.30$  &  $+0.21$  &  $+0.18$  &  $+0.13$  &  $+0.15$  &  $+0.54$  &  $+0.39$  \\
\ion{Si}{I}   &  $6142.494$  &  $5.62$  &  $-1.50$  &  $+0.24$  &  $+0.22$  &  ---      &  $+0.50$  &  $+0.02$  &  $+0.29$  \\
\ion{Si}{I}   &  $6145.020$  &  $5.61$  &  $-1.45$  &  $+0.49$  &  $+0.19$  &  ---      &  ---      &  $+0.23$  &  $+0.42$  \\
\ion{Si}{I}   &  $6155.142$  &  $5.62$  &  $-0.85$  &  $+0.05$  &  $+0.40$  &  $+0.20$  &  $+0.30$  &  $+0.09$  &  $+0.25$  \\
\ion{Si}{I}   &  $6237.328$  &  $5.61$  &  $-1.01$  &  $+0.43$  &  $+0.48$  &  $+0.31$  &  $+0.29$  &  $+0.43$  &  $+0.48$  \\
\ion{Si}{I}   &  $6243.823$  &  $5.61$  &  $-1.30$  &  $+0.53$  &  $+0.46$  &  ---      &  $+0.42$  &  $+0.46$  &  $+0.06$  \\
\ion{Si}{I}   &  $6414.987$  &  $5.87$  &  $-1.13$  &  $+0.12$  &  $+0.45$  &  $+0.42$  &  $+0.51$  &  $+0.67$  &  $+0.64$  \\
\ion{Si}{I}   &  $6721.844$  &  $5.86$  &  $-1.17$  &  $+0.60$  &  $+0.43$  &  $+0.52$  &  $+0.49$  &  $+0.40$  &  $+0.31$  \\
\ion{Ca}{I}   &  $5601.277$  &  $2.53$  &  $-0.52$  &  $-0.33$  &  $+0.07$  &  ---      &  ---      &  ---      &  $+0.22$  \\   
\ion{Ca}{I}   &  $5867.562$  &  $2.93$  &  $-1.55$  &  $+0.50$  &  $+0.02$  &  $+0.49$  &  $+0.40$  &  $+0.41$  &  $+0.40$  \\ 
\ion{Ca}{I}   &  $6156.030$  &  $2.52$  &  $-2.39$  &  ---      &  ---      &  ---      &  $+0.40$  &  $+0.56$  &  $+0.44$  \\ 
\ion{Ca}{I}   &  $6161.295$  &  $2.51$  &  $-1.02$  &  $+0.26$  &  ---      &  $+0.50$  &  $-0.10$  &  $-0.09$  &  $+0.48$  \\ 
\ion{Ca}{I}   &  $6166.440$  &  $2.52$  &  $-0.90$  &  $+0.37$  &  $+0.53$  &  $-0.39$  &  $+0.30$  &  $+0.27$  &  $+0.11$  \\
\ion{Ca}{I}   &  $6169.044$  &  $2.52$  &  $-0.54$  &  $+0.45$  &  $+0.43$  &  ---      &  $+0.00$  &  $+0.11$  &  $+0.28$  \\ 
\ion{Ca}{I}   &  $6169.564$  &  $2.52$  &  $-0.27$  &  $+0.55$  &  $+0.44$  &  ---      &  ---      &  $+0.15$  &  $+0.42$  \\ 
\ion{Ca}{I}   &  $6439.080$  &  $2.52$  &  $+0.30$  &  $+0.24$  &  $+0.55$  &  ---      &  ---      &  ---      &  $+0.50$  \\   
\ion{Ca}{I}   &  $6455.605$  &  $2.52$  &  $-1.35$  &  $+0.47$  &  $+0.48$  &  $+0.43$  &  $+0.10$  &  $+0.40$  &  $+0.47$  \\ 
\ion{Ca}{I}   &  $6464.679$  &  $2.52$  &  $-2.10$  &  ---      &  ---      &  ---      &  $+0.49$  &  $+0.37$  &  $+0.55$  \\ 
\ion{Ca}{I}   &  $6493.788$  &  $2.52$  &  $-2.44$  &  $-0.07$  &  $+0.14$  &  ---      &  ---      &  ---      &  $-0.10$  \\   
\ion{Ca}{I}   &  $6499.654$  &  $2.52$  &  $-0.85$  &  $+0.36$  &  $+0.58$  &  $+0.15$  &  ---      &  $+0.20$  &  $+0.43$  \\ 
\ion{Ca}{I}   &  $6572.779$  &  $0.00$  &  $-4.32$  &  ---      &  ---      &  $-0.16$  &  $+0.20$  &  $+0.32$  &  $+0.08$  \\ 
\ion{Ca}{I}   &  $6717.687$  &  $2.71$  &  $-0.61$  &  $+0.46$  &  ---      &  $-0.23$  &  $-0.10$  &  $+0.33$  &  $+0.43$  \\ 
\ion{Ti}{I}   &  $5689.459$  &  $2.29$  &  $-0.44$  &  $+0.39$  &  $+0.39$  &  $+0.42$  &  $+0.49$  &  $+0.44$  &  $+0.58$  \\
\ion{Ti}{I}   &  $5866.449$  &  $1.07$  &  $-0.84$  &  $+0.36$  &  $+0.51$  &  $+0.12$  &  $+0.09$  &  $+0.48$  &  $+0.29$  \\
\ion{Ti}{I}   &  $5922.108$  &  $1.05$  &  $-1.46$  &  ---      &  $+0.43$  &  $+0.32$  &  $+0.40$  &  $+0.27$  &  $+0.35$  \\
\ion{Ti}{I}   &  $5941.750$  &  $1.05$  &  $-1.50$  &  $+0.49$  &  $+0.28$  &  $+0.50$  &  $+0.30$  &  $+0.23$  &  $+0.35$  \\
\ion{Ti}{I}   &  $5965.825$  &  $1.88$  &  $-0.42$  &  $+0.54$  &  $+0.53$  &  $+0.47$  &  $+0.20$  &  $+0.30$  &  $+0.33$  \\
\ion{Ti}{I}   &  $5978.539$  &  $1.87$  &  $-0.53$  &  $+0.02$  &  $+0.36$  &  $+0.46$  &  $+0.60$  &  $+0.56$  &  $+0.13$  \\
\ion{Ti}{I}   &  $6064.623$  &  $1.05$  &  $-1.94$  &  ---      &  $+0.58$  &  $+0.48$  &  ---      &  $+0.44$  &  $+0.35$  \\
\ion{Ti}{I}   &  $6091.169$  &  $2.27$  &  $-0.42$  &  $+0.36$  &  $+0.43$  &  $+0.49$  &  $+0.40$  &  $+0.49$  &  $+0.33$  \\
\ion{Ti}{I}   &  $6126.214$  &  $1.07$  &  $-1.43$  &  $+0.46$  &  $+0.57$  &  $+0.36$  &  $+0.00$  &  $+0.33$  &  $+0.22$  \\
\ion{Ti}{I}   &  $6258.110$  &  $1.44$  &  $-0.36$  &  $+0.11$  &  $+0.31$  &  $+0.22$  &  $+0.00$  &  $-0.08$  &  $-0.22$  \\  
\ion{Ti}{I}   &  $6261.106$  &  $1.43$  &  $-0.48$  &  $+0.57$  &  $+0.45$  &  $+0.13$  &  $+0.00$  &  $-0.04$  &  $+0.06$  \\  
\ion{Ti}{I}   &  $6303.767$  &  $1.44$  &  $-1.57$  &  $+0.56$  &  $+0.56$  &  ---      &  $+0.20$  &  $+0.57$  &  $+0.39$  \\
\ion{Ti}{I}   &  $6312.240$  &  $1.46$  &  $-1.60$  &  ---      &  ---      &  $+0.09$  &  $+0.50$  &  ---      &  $+0.26$  \\
\ion{Ti}{I}   &  $6336.113$  &  $1.44$  &  $-1.74$  &  ---      &  $+0.25$  &  ---      &  ---      &  ---      &  $+0.56$  \\
\ion{Ti}{I}   &  $6508.150$  &  $1.43$  &  $-2.05$  &  ---      &  $+0.60$  &  ---      &  ---      &  ---      &  $+0.28$  \\
\ion{Ti}{I}   &  $6554.238$  &  $1.44$  &  $-1.22$  &  $-0.10$  &  $+0.47$  &  $+0.33$  &  $+0.20$  &  $+0.37$  &  $+0.38$  \\
\ion{Ti}{I}   &  $6556.077$  &  $1.46$  &  $-1.07$  &  $+0.25$  &  ---      &  $+0.42$  &  $+0.40$  &  $+0.46$  &  $+0.59$  \\
\ion{Ti}{I}   &  $6599.113$  &  $0.90$  &  $-2.09$  &  $+0.52$  &  $+0.50$  &  $+0.46$  &  $+0.60$  &  $+0.68$  &  $+0.40$  \\
\ion{Ti}{I}   &  $6743.127$  &  $0.90$  &  $-1.73$  &  $+0.39$  &  $+0.47$  &  $+0.10$  &  $+0.40$  &  $+0.49$  &  $+0.52$  \\
\ion{Ti}{II}  &  $5418.751$  &  $1.58$  &  $-2.13$  &  ---      &  ---      &  $-0.23$  &  ---      &  $+0.20$  &  $+0.27$  \\
\ion{Ti}{II}  &  $6491.580$  &  $2.06$  &  $-2.10$  &  $+0.18$  &  $+0.38$  &  $+0.23$  &  $-0.10$  &  $+0.00$  &  $+0.41$  \\
\ion{Ti}{II}  &  $6559.576$  &  $2.05$  &  $-2.35$  &  $+0.14$  &  $+0.26$  &  $+0.48$  &  $+0.10$  &  $+0.26$  &  ---      \\
\ion{Ti}{II}  &  $6606.970$  &  $2.06$  &  $-2.85$  &  $+0.26$  &  $+0.39$  &  $+0.02$  &  $+0.40$  &  $+0.36$  &  $+0.23$  \\  
\hline
\ion{Y}{I}    &  $6435.004$  &  $0.07$  &  $-0.82$  &  $+0.02$  &  $+0.44$  &  $+1.12$  &  $+0.78$  &  $+0.89$  &  $-0.01$ \\
\ion{Y}{II}   &  $6795.414$  &  $1.74$  &  $-1.19$  &  $+0.33$  &  $+0.23$  &  $+0.48$  &  $+0.84$  &  $+0.57$  &  $+0.09$ \\
\ion{Zr}{I}   &  $6127.475$  &  $0.15$  &  $-1.06$  &  $+0.71$  &  $+0.74$  &  $+0.58$  &  $+0.60$  &  $+0.85$  &  $+0.29$ \\
\ion{Zr}{I}   &  $6134.585$  &  $0.00$  &  $-1.42$  &  $+0.86$  &  $+0.37$  &  $+0.84$  &   ---     &  $+0.33$  &  $+0.48$ \\
\ion{Zr}{I}   &  $6140.535$  &  $0.52$  &  $-1.60$  &   ---     &  $+0.86$  &   ---     &   ---     &  $+0.95$  &  $+0.92$ \\
\ion{Zr}{I}   &  $6143.252$  &  $0.07$  &  $-1.10$  &  $+0.71$  &  $+0.75$  &  $+0.54$  &  $+0.63$  &  $+0.84$  &  $-0.04$ \\
\ion{Ba}{II}  &  $5853.675$  &  $0.60$  &  $-1.10$  &   ---     &  $+0.52$  &   ---     &   ---     &   ---     &  $+0.36$ \\
\ion{Ba}{II}  &  $6496.897$  &  $0.60$  &  $-0.32$  &   ---     &  $+0.65$  &   ---     &  $+0.23$  &   ---     &  $+0.62$ \\
\ion{La}{II}  &  $6172.721$  &  $0.13$  &  $-2.25$  &  $+0.72$  &  $+0.03$  &  $+0.86$  &  $+0.78$  &  $+0.81$  &  $+0.32$ \\
\ion{La}{II}  &  $6262.287$  &  $0.40$  &  $-1.60$  &  $+0.55$  &  $+0.30$  &   ---     &   ---     &  $+0.37$  &  $+0.16$ \\
\ion{La}{II}  &  $6296.079$  &  $1.25$  &  $-0.84$  &  $+0.37$  &   ---     &   ---     &   ---     &   ---     &  $+0.19$ \\
\ion{La}{II}  &  $6320.376$  &  $0.17$  &  $-1.56$  &  $+0.37$  &  $+0.29$  &  $+0.19$  &  $+0.52$  &  $+0.79$  &  $+0.21$ \\
\ion{La}{II}  &  $6390.477$  &  $0.32$  &  $-1.41$  &  $+0.31$  &  $+0.10$  &  $+0.67$  &  $+0.77$  &  $+0.75$  &  $+0.30$ \\
\ion{Eu}{II}  &  $6437.640$  &  $1.32$  &  $-0.32$  &  $+0.55$  &  $+0.50$  &  $+0.62$  &  $+0.65$  &  $+0.77$  &  $+0.57$ \\
\ion{Eu}{II}  &  $6645.064$  &  $1.38$  &  $+0.12$  &  $+0.31$  &  $+0.12$  &  $+0.37$  &  $+0.82$  &  $+0.72$  &  $+0.59$ \\ 
\\ \hline \hline \\            
\end{longtable} 
\twocolumn
